Overlap matrix concentration in optimal Bayesian inference

We consider models of Bayesian inference of signals with vectorial components of finite dimensionality. We show that, under a proper perturbation, these models are replica symmetric in the sense that the overlap matrix concentrates. The overlap matrix is the order parameter in these models and is directly related to error metrics such as minimum mean-square errors. Our proof is valid in the optimal Bayesian inference setting. This means that it relies on the assumption that the model and all its hyper-parameters are known so that the posterior distribution can be written exactly. Examples of important problems in high-dimensional inference and learning to which our results apply are low-rank tensor factorization, the committee machine neural network with a finite number of hidden neurons in the teacher-student scenario, or multi-layer versions of the generalized linear model.

==> sections/Lconc_detailedK.tex <==
\section{Concentration of the matrix ${\cal L}$}
%
The goal of this appendix is to prove Theorem \ref{prop:Lconc}. Recall that we denote $C(\theta)$ a generic positive numerical constant depending only on the parameters $\theta$, e.g. $C(S)$ depends only on the prior support $S$. The proof of Proposition \ref{prop:Lconc} is broken in two parts, using the decomposition
%
\begin{align*}
\mathbb{E}\big\langle \|\mathcal{L} - \mathbb{E}\langle \mathcal{L}\rangle\|^2_{\rm F}\big\rangle
& = 
\mathbb{E}\big\langle \|\mathcal{L} - \langle \mathcal{L}\rangle\|^2_{\rm F}\big\rangle
+ 
\mathbb{E}\big[\|\langle \mathcal{L}\rangle - \mathbb{E}\langle \mathcal{L}\rangle\|^2_{\rm F}\big]\,.
\end{align*}
%
Thus it suffices to prove the two following propositions. The first one expresses concentration w.r.t.\ the posterior distribution (or ``thermal fluctuations'') and is a direct consequence of concavity properties of the average free energy and the Nishimori identity. 

We recall the main hypothesis used 
%
\begin{proposition}[Thermal fluctuations]\label{thermal-fluctuations}
	Let $\beta_s>\beta_K>0$ verifying \ $6\beta_K+\beta_s<1$. Consider sequences $(s_n=n^{-\beta_s})\in(0,1]^\mathbb{N}$ and $(K_n=\floor*{K_* n^{\beta_K}})\in\mathbb{N}^{\mathbb{N}}$, with $K_*\in\mathbb{N}$. There exists a positive constant $C(S)$ s.t.
	\begin{align*}
		s_n^{-K_n^2}\int_{{\cal D}_{n,K_n}} d\lambda\, 
  \mathbb{E} \big\langle \|\mathcal{L} - \langle \mathcal{L}\rangle\|_{\rm F}^2 \big\rangle  \le C(S)\frac{K_n^6}{s_nn}\,.
	\end{align*}
\end{proposition}
\begin{proof}
By direct computation we have for any $(l,l')\in\{1,\ldots,K\}^2$
\begin{align}
\mathbb{E}\big\langle (\mathcal{L}_{ll'} - \langle \mathcal{L}_{ll'} \rangle)^2\big\rangle
& = 
-\frac{1}{n}\frac{d^2f_n}{d\lambda_{ll'}^2}
+\frac{1}{n} \mathbb{E}\Big\langle\frac{d{\cal L}_{ll'}}{d\lambda_{ll'}} \Big\rangle \,.
\label{directcomputation}
\end{align}
%
Computing the derivative of $\mathcal{L}_{ll'}$ and using $-2\big(\frac{d\lambda^{1/2}}{d\lambda_{ll'}}\big)^2=\lambda^{1/2}\frac{d^2\lambda^{1/2}}{d\lambda_{ll'}^2}+\frac{d^2\lambda^{1/2}}{d\lambda_{ll'}^2}\lambda^{1/2}$ which follows from \eqref{57} we find, using \eqref{66} and similar computations as \eqref{76}--\eqref{77_bis},
%
\begin{align}
\Big|\frac{1}{n}\mathbb{E}\Big\langle \frac{d\mathcal{L}_{ll'}}{d\lambda_{ll'}} \Big\rangle\Big| =\Big|\frac1{n^2}\sum_{i=1}^n\EE\Big[\Big\langle x_i^\intercal\Big(\frac{d\lambda^{1/2}}{d\lambda_{ll'}}\Big)^2x_i\Big\rangle-\langle x_i^\intercal\rangle \Big(\frac{d\lambda^{1/2}}{d\lambda_{ll'}}\Big)^2\langle x_i\rangle\Big]\Big|\le C(S)\frac{K^4}{s_nn}\,.\label{44}
\end{align}
%
The last inequality is obtained by bounding the entries of the square-root matrix $\lambda\in{\cal D}_{n,K}$ as follows. By definition of the square-root matrix, and the fact that it is symmetric, we can write that the diagonal entry $\lambda_{ll}=\sum_{k=1}^K (\lambda^{1/2}_{lk})^2\le (2K+1)s_n$ where the last inequality follows from the fact that $\lambda\in{\cal D}_{n,K}$. As each term in this sum is non-negative we can assert $(\lambda^{1/2}_{lk})^2\le (2K+1)s_n$. Therefore all entries of the matrix $\lambda^{1/2}$ are ${\cal O}(\sqrt{Ks_n})$. We can conclude that the entries of $\frac{d\lambda^{1/2}}{d\lambda_{ll'}}$ are ${\cal O}(\sqrt{K/s_n})$, and those of $(\frac{d\lambda^{1/2}}{d\lambda_{ll'}})^2$ are ${\cal O}(K^2/s_n)$). 

We integrate the equality \eqref{directcomputation} over $\lambda_{ll'}\in (a_n,b_n)=(s_n,2s_n)$ if $l\neq l'$ or $\lambda_{ll}\in (a_n,b_n)=(2Ks_n, (2K+1)s_n)$ else, and obtain
\begin{align*}
\int_{a_n}^{b_n} d\lambda_{ll'}\, \mathbb{E}\big\langle (\mathcal{L}_{ll'} - \langle \mathcal{L}_{ll'} \rangle)^2\big\rangle
& \leq 
- \frac{1}{n}\int_{a_n}^{b_n} d\lambda_{ll'} \,\frac{d^2f_{n}}{d\lambda_{ll'}^2} + C(S)\frac{K^4}{n}
\nonumber \\ &
=
\frac{1}{n}\Big(\frac{df_{n}}{d\lambda_{ll'}}(\lambda_{ll'}=a_n) 
- \frac{df_{n}}{d\lambda_{ll'}}(\lambda_{ll'}=b_n)\Big)+ C(S)\frac{K^4}{n}\,.
\end{align*}
%
We have $|d f_{n}/d\lambda_{ll'}| \le |\mathbb{E}\langle R_{ll'}\rangle|\le S^2$ from \eqref{80}, \eqref{80_ll} so the first term is certainly smaller in absolute value than $2S^2/n$. Therefore
%
\begin{align*}
\int_{a_n}^{b_n} d\lambda_{ll'}\, \mathbb{E}\big\langle (\mathcal{L}_{ll'} - \langle \mathcal{L}_{ll'} \rangle)^2\big\rangle\le2S^2\frac{1}{n}+C(S)\frac{K^4}{n}=C(S)\frac{K^4}{n}\,.	
\end{align*}
%
In the last equality, the constants $C(S)$ are different. We now average this inequality w.r.t. to the remaining $K^2-1$ matrix elements of $\lambda\in{\cal D}_{n,K}$, where the set ${\cal D}_{n,K}$ is defined by \eqref{DnK}. This yields 
%
\begin{align*}
s_n^{-K^2}\int_{{\cal D}_{n,K}} d\lambda\, \mathbb{E}\big\langle (\mathcal{L}_{ll'} - \langle \mathcal{L}_{ll'} \rangle)^2\big\rangle\le C(S)\frac{K^4}{s_nn}\,.	
\end{align*}
%
Summing all $K^2$ fluctuations for the various couples $(l,l')$ yields the desired bound. 
\end{proof}
%
The second proposition expresses the concentration w.r.t.\ the quenched disorder variables
and is a consequence of the concentration of the free energy onto its average (w.r.t. the quenched variables).
%
\begin{proposition}[Quenched fluctuations]\label{disorder-fluctuations}
	Let $0<\beta_s/7<\beta_K<\beta_s<1/6$. Let the sequences $(s_n=n^{-\beta_s})\in(0,1]^\mathbb{N}$ and $(K_n=n^{\beta_K})\in\mathbb{N}^{\mathbb{N}}$. There exists a positive constant $C(C_f,S)$ s.t. 
	\begin{align*}
		s_n^{-K^2}\int_{{\cal D}_{n,K}} d\lambda\, 
  \mathbb{E} \big[\|\langle \mathcal{L}\rangle-\EE\langle \mathcal{L}\rangle \|_{\rm F}^2 \big]  \le C(C_f,K,S)\frac{1}{s_n^{4/3}n^{1/3}}\,.
	\end{align*}
\end{proposition}
%
\begin{proof}
Let us define the non-averaged free energy: $F_{n}(\lambda)= F_{n}(\lambda;\widetilde Y,Y,\theta,h)\equiv-\frac{1}{n} \ln {\cal Z}_n(\widetilde Y,Y,\theta,h)$, so that the averaged one given by \eqref{av_f} is simply $f_n(\lambda)=\EE \,F_{n}(\lambda)$.
We have the following identities: for any given realisation of the quenched disorder and any fixed $(l,l')\in\{1,\ldots,K\}^2$ 
\begin{align}
 \frac{dF_{n}(\lambda)}{d\lambda_{ll'}}  &= \langle \mathcal{L}_{ll'} \rangle \,,\nonumber\\
 %
 \frac{1}{n}\frac{d^2F_{n}(\lambda)}{d\lambda_{ll'}^2}  &= -\big\langle (\mathcal{L}_{ll'}  - \langle \mathcal{L}_{ll'} \big\rangle)^2\rangle-
 \frac{1}{n^2}\sum_{i=1}^n  \langle x_i^\intercal\rangle \frac{d^2\lambda^{1/2}}{d\lambda_{ll'}^2} Z_i \,.\label{second-derivative}
\end{align}
We obtain the same identities for $f_n(\lambda)=\EE \,F_{n}(\lambda)$ but with an average $\EE$ over the quenched disorder (recall e.g. \eqref{80}). The thermal fluctuations of $\cal L$ are almost directly equal to the the second derivative of $-\frac1n F_n(\lambda)$ as seen from \eqref{second-derivative}, up to a lower order term that we consider now. We have 
%
\begin{align}
\langle x_i^\intercal\rangle \frac{d^2\lambda^{1/2}}{d\lambda_{ll'}^2} Z_i=\sum_{kk'}	\langle x_{ik}\rangle \Big(\frac{d^2\lambda^{1/2}}{d\lambda_{ll'}^2}\Big)_{kk'} Z_{ik'}\le S D_n(K) K\sum_{k'}|Z_{ik'}|\label{51}
\end{align}
%
where $D_n(K)\equiv \max_{\{kk',ll'\}}\big|\big(\frac{d^2\lambda^{1/2}}{d\lambda_{ll'}^2}\big)_{kk'}\big|=s_n^{-3/2}C(K)$. Let us evaluate the scaling in $K$ of $D_n$. As explained below \eqref{44} all entries of the matrix $\lambda^{1/2}$ are ${\cal O}(\sqrt{Ks_n})$. Therefore $D_n(K) \le C s_n^{-3/2}\sqrt{K}$ for some constant $C$ independent of $K$ or $n$. Therefore the following function of $\lambda_{ll'}$
\begin{align}\label{new-free}
 &F_{n,ll'}(\lambda_{ll'}) \equiv F_{n}(\lambda) - \frac{\lambda_{ll'}^2}{2} CS\Big(\frac{K}{s_n}\Big)^{3/2}\frac1n\sum_{i,k'=1}^{n,K}|Z_{ik'}|
\end{align}
%
is concave by construction, because thanks to 
\eqref{second-derivative}, \eqref{51} we see that the second derivative of $F_{n,ll'}(\lambda_{ll'})$ is negative (for a sufficiently large constant $C$). Obviously its average
\begin{align}\label{new-free-2}
 f_{n,ll'}(\lambda_{ll'}) \equiv \mathbb{E} \,F_{n,ll'}(\lambda_{ll'})= f_{n}(\lambda)  -\frac{\lambda_{ll'}^2}{2} CS\Big(\frac{K}{s_n}\Big)^{3/2}\frac1n\sum_{i,k'=1}^{n,K}\EE\,|Z_{ik'}|
\end{align}
is concave too.
Concavity then allows to use the following standard Lemma (see e.g. \cite{BarbierM17a,barbier2017phase} for a proof):
%
\begin{lemma}[A bound for concave functions]\label{lemmaConvexity}
Let $G(x)$ and $g(x)$ be concave functions. Let $\delta>0$ and define $C^{-}_\delta(x) \equiv g'(x-\delta) - g'(x) \geq 0$ and $C^{+}_\delta(x) \equiv g'(x) - g'(x+\delta) \geq 0$. Then
\begin{align*}
|G'(x) - g'(x)| \leq \delta^{-1} \sum_{u \in \{x-\delta,\, x,\, x+\delta\}} |G(u)-g(u)| + C^{+}_\delta(x) + C^{-}_\delta(x)\,.
\end{align*}
\end{lemma}
%
First, from \eqref{new-free}, \eqref{new-free-2} we have 
\begin{align}\label{fdiff}
 F_{n,ll'}(\lambda_{ll'}) - f_{n,ll'}(\lambda_{ll'}) = F_{n}(\lambda) - f_{n}(\lambda) - \frac{\lambda_{ll'}^2}{2} CS\Big(\frac{K}{s_n}\Big)^{3/2} A_n 
\end{align} 
with $A_n \equiv \frac{1}{n}\sum_{i,k'=1}^{n,K} (\vert Z_{ik'}\vert -\mathbb{E}\,\vert  Z_{ik'}\vert)$.
Second, we obtain for the $\lambda_{ll'}$-derivatives difference
\begin{align}\label{derdiff}
 F_{n,ll'}'(\lambda_{ll'}) - f_{n,ll'}'(\lambda_{ll'}) = 
\langle \mathcal{L}_{ll'} \rangle-\mathbb{E}\langle \mathcal{L}_{ll'} \rangle -\lambda_{ll'}CS\Big(\frac{K}{s_n}\Big)^{3/2}A_n \,.
\end{align}
From \eqref{fdiff} and \eqref{derdiff} it is then easy to show that Lemma \ref{lemmaConvexity} applied to $G(x) \to F_{n,ll'}(\lambda_{ll'})$ and $g(x)\to f_{n,ll'}(\lambda_{ll'})$ with $x\to \lambda_{ll'}$ gives
\begin{align}\label{usable-inequ}
\vert \langle \mathcal{L}_{ll'}\rangle - \mathbb{E}\langle \mathcal{L}_{ll'}\rangle\vert&\leq 
\delta^{-1} \sum_{u\in \{\lambda_{ll'} -\delta,\, \lambda_{ll'},\, \lambda_{ll'}+\delta\}}
 \big(\vert F_{n}(u) - f_{n}(u) \vert + \frac{u^2}{2}CS\Big(\frac{K}{s_n}\Big)^{3/2}\vert A_n \vert \big)\nonumber\\
 &\qquad
  + C_\delta^+(\lambda_{ll'}) + C_\delta^-(\lambda_{ll'}) + \big((2K+1)\mathbf{1}(l'=l)+2\mathbf{1}(l'\neq l)\big)CS\Big(\frac{K^3}{s_n}\Big)^{1/2}\vert A_n\vert
\end{align}
where we used $\lambda_{ll'}\le (2K+1)s_n$ for any $l\neq l'\in\{1,\ldots,K\}$ and $\lambda_{ll}\le 2s_n$ as $\lambda\in {\cal D}_{n,K}$. $\mathbf{1}(\cdot)$ is the indicator function. Moreover $C_\delta^-(\lambda_{ll'})\equiv f_{n,ll'}'(\lambda_{ll'}-\delta)-f_{n,ll'}'(\lambda_{ll'})\ge 0$ 
and $C_\delta^+(\lambda_{ll'})\equiv f_{n,ll'}'(\lambda_{ll'})-f_{n,ll'}'(\lambda_{ll'}+\delta)\ge 0$. Note that $\delta$ will be chosen small enough so that when $\lambda_{ll'}$ is varied by $\pm \delta$ the matrix $\lambda$ remains in the set ${\cal D}_{n,K}$. Remark that by independence of the noise variables $\mathbb{E}[A_n^2]  \le  (1-2/\pi) K/n$. We square the identity \eqref{usable-inequ} and take its expectation. Let us denote $U_{ll'}(K)\equiv(2K+1)\mathbf{1}(l'=l)+2\mathbf{1}(l'\neq l)$. Then using $(\sum_{i=1}^pv_i)^2 \le p\sum_{i=1}^pv_i^2$ by convexity, again that $\lambda\in{\cal D}_{n,K}$, as well as the free energy concentration hypothesis ?? (all positive numerical constants are absorbed in the generic positive constants $C(\cdot)$),
%
\begin{align}\label{intermediate}
 \mathbb{E}\big[(\langle \mathcal{L}_{ll'}\rangle - \mathbb{E}\langle \mathcal{L}_{ll'}\rangle)^2\big]
 &
 \leq \, 
  \frac{C_{f,n}}{n\delta^2} + \big\{U_{ll'}(K)s_n+\delta\big\}^4 C(S)\frac{K^4}{n\delta^2s_n^3}  \nn
  &\qquad \qquad+ C_\delta^+(\lambda_{ll'})^2 + C_\delta^-(\lambda_{ll'})^2+U_{ll'}(K)^2C(S)\frac{K^4}{s_nn}\, .
\end{align}
Recall $|C_\delta^\pm(\lambda_{ll'})|=|f'_{n,ll'}(\lambda_{ll'}\pm\delta)-f'_{n,ll'}(\lambda_{ll'})|$. We have (here $Z\sim{\cal N}(0,1)$)
\begin{align}
|f'_{n,ll'}(\lambda_{ll'})| = \Big|\EE\langle {\cal L}_{ll'}\rangle -\lambda_{ll'}CS\Big(\frac{K}{s_n}\Big)^{3/2}\EE\,|Z|\Big|  \leq C(S)U_{ll'}(K)\Big(\frac{K^3}{s_n}\Big)^{1/2}\label{boudfprime}	
\end{align}
using \eqref{80}, \eqref{80_ll} to assess that $\EE\langle {\cal L}_{ll'}\rangle\le S^2$. Therefore we have the following crude bound $$|C_\delta^\pm(\lambda_{ll'})|\le C(S)U_{ll'}(K)\Big(\frac{K^3}{s_n}\Big)^{1/2}\,.$$ Let $(a_n,b_n)=(s_n,2s_n)$ if $l\neq l'$ or $(a_n,b_n)=(2Ks_n, (2K+1)s_n)$ else. We reach
%
\begin{align*}
 \int_{a_n}^{b_n} &d\lambda_{ll'}\,\big\{C_\delta^+(\lambda_{ll'})^2 + C_\delta^-(\lambda_{ll'})^2\big\}\nn
 %
  &\leq  C(S)U_{ll'}(K)\Big(\frac{K^3}{s_n}\Big)^{1/2}
 \int_{{a_n}}^{{b_n}} d\lambda_{ll'}\, \big\{C_\delta^+(\lambda_{ll'}) + C_\delta^-(\lambda_{ll'})\big\}
 \nonumber \\ 
&= 
C(S)U_{ll'}(K)\Big(\frac{K^3}{s_n}\Big)^{1/2}\big[\big(f_{n,ll'}(a_n+\delta) - f_{n,ll'}(a_n-\delta)\big)+ \big(f_{n,ll'}(b_n-\delta) - f_{n,ll'}(b_n+\delta)\big)\big]\,.
\end{align*}
%
The mean value theorem and \eqref{boudfprime} 
imply $$|f_{n,ll'}(\lambda_{ll'}-\delta) - f_{n,ll'}(\lambda_{ll'}+\delta)|\le \delta C(S)U_{ll'}(K)\Big(\frac{K^3}{s_n}\Big)^{1/2}\,.$$ Therefore
%
\begin{align*}
 \int_{a_n}^{b_n} d\lambda_{ll'}\, \big\{C_\delta^+(\lambda_{ll'})^2 + C_\delta^-(\lambda_{ll'})^2\big\}\leq   C(S)U_{ll'}(K)^2K^3\frac{\delta}{s_n}\,.
\end{align*}
%
Thus, integrating \eqref{intermediate} over $\lambda_{ll'}\in (a_n, b_n)$ and choosing $\delta=\delta_n$ s.t. $\delta_n/s_n\to 0$ yields
\begin{align*}
 \int_{a_n}^{b_n} d\lambda_{ll'}\, 
 \mathbb{E}\big[(\langle \mathcal{L}_{ll'}\rangle - \mathbb{E}\langle \mathcal{L}_{ll'}\rangle)^2\big]&\leq C_{f,n}\frac{s_n}{n\delta_n^2} + U_{ll'}(K)^4 C(S)\frac{K^4s_n^2}{n\delta_n^2} \nn
 &\qquad\qquad\qquad+ C(S)U_{ll'}(K)^2\frac{K^3\delta_n}{s_n}+ U_{ll'}(K)^2C(S)\frac{K^4}{n}\,.
\end{align*}
%
We average this identity over the remaining $K^2-1$ entries of $\lambda\in{\cal D}_{n,K}$, and summing the $K^2$ fluctuations for the various $(l,l')$ couples using (for any $p\ge 1$)
%
\begin{align}
	\sum_{l,l'=1}^KU_{ll'}^p(K)=K(2K+1)^p+K(K-1)2^p \le C (K^{p+1}+K^2)=CK^{p+1}\,,
\end{align}
%	
we reach
%
\begin{align*}
 s_n^{-K^2}\int_{{\cal D}_{n,K}} d\lambda\, 
  \mathbb{E} \big[\|\langle \mathcal{L}\rangle-\EE\langle \mathcal{L}\rangle \|_{\rm F}^2 \big]&\leq C_{f,n}\frac{K^2}{n\delta_n^2} + C(S)\frac{K^9s_n}{n\delta_n^2} + C(S)\frac{K^6\delta_n}{s_n^2}+ C(S)\frac{K^7}{s_nn}\,.
\end{align*}
%
When $K=K_n=n^{\beta_K}$ with $\beta_s/7<\beta_K<\beta_s$ the second term on the r.h.s. dominates the first one. Therefore in order to optimize the bound we need to choose $\delta_n$ s.t. the scaling of the second and third terms are the same, i.e. $n^{9\beta_K-\beta_s-1}\delta_n^{-2}=n^{6\beta_K+2\beta_s}\delta_n$ which selects $\delta_n  = n^{\beta_K-\beta_s-1/3}$ (it indeed verifies $\delta_n\to 0_+$ and $\delta_n/s_n = n^{\beta_K-1/3}\to 0_+$). The desired result is then obtaind when keeping only the dominant terms.
\end{proof}

==> sections/alternative.tex <==
\section{Alternative approach}
%
\subsection{The generalized low-rank tensor perturbation}
%
In order for the Nishimori identity to apply, one must be careful in designing a perturbation Hamiltonian. A proper perturbation must be an Hamiltonian itself coming from an inference problem (sometimes refered to as a ``side channel''). Let us denote the generalized index $I\equiv \{i_1,\ldots,i_p\}\in\{1,\ldots,n\}^p$ for any integer $p\ge 1$, and a generalized variable $x^{(a)}_I\equiv x_{i_1}^{(a)}\ldots x_{i_p}^{(a)}\in\mathbb{R}^K$ where the product is an Hadamard (componentwise) product, and its $k$-th component $x_{Ik}^{(a)} \equiv x_{i_1k}^{(a)}\ldots x_{i_pk}^{(a)}$. Let $\lambda=(\lambda_k)\in\{-1,0,1\}^K$, where $\lambda_k^2$ plays the role of a rank-dependent signal-to-noise ratio (SNR). Consider the Hamiltonian coming from the following ``generalized low-rank tensor'' observation channel (here $Y_I$ is a scalar):
%
\begin{align}
Y_I=\gamma_nn^{\frac{1-p}{2}}\lambda^\intercal X_{I} + Z_I\,, \qquad I\in\{1,\ldots,n\}^p\,,	
\end{align}
where $(Z_I)=(Z_{i_1\ldots i_p})$ are i.i.d. standard Gaussians for different indices, $\gamma_n\equiv s_n\beta$ with $\beta\in[1,2]$, $(s_n)$ a sequence going to zero and $X_I\sim P_0^{\otimes p}$ is still the planted signal. Here the signal-tensor observed through the noisy Gaussian channel is of order-$p$ and rank-$K$. The perturbation Hamiltonian is in this case 
%
\begin{align}
	{\cal H}_{\rm pert}^{(p)}(x;Y(X,Z))&\equiv -\sum_{I}\Big( \gamma_nn^{\frac{1-p}{2}}Y_I \lambda^\intercal x_{I}-\frac12\gamma_n^2n^{1-p}(\lambda^\intercal x_{I})^2\Big) \nn
	% &= -\sum_{I} \Big(\gamma_n^2n^{1-p}\sum_{k,k'}\lambda_k\lambda_{k'}X_{Ik}x_{Ik'} + \gamma_nn^{\frac{1-p}{2}}\widetilde g_I \sum_{k}\lambda_k x_{Ik} -\frac12\gamma_n^2n^{1-p}\sum_{k,k'}\lambda_k\lambda_{k'}x_{Ik}x_{Ik'}\Big) \nn
	%
	&= -\sum_{I} \Big(\gamma_n^2n^{1-p}\lambda^\intercal X_{I}x_{I}^\intercal \lambda + \gamma_nn^{\frac{1-p}{2}}Z_I x_{I}^\intercal \lambda -\frac12\gamma_n^2n^{1-p}\lambda^\intercal x_{I}x_{I}^\intercal \lambda\Big) \nn
	%
	&= -\Big(\gamma_n^2nQ_{0,1}^{(p)} + \gamma_nn^{\frac{1-p}{2}}\sum_IZ_I x_{I}^\intercal \lambda -\frac12\gamma_n^2nQ_{1,1}^{(p)}\Big)\,. \label{one_inf}
\end{align}
%
The overlap matrix and generalized overlap are, respectively,
%
\begin{align}
	R_{a,b}&=(R_{a,b}^{k,k'})_{k,k'\le K}\equiv \Big(\frac{1}{n}\sum_{i} x_{ik}^{(a)} x_{ik'}^{(b)}\Big)_{k,k'\le K}= \frac{1}{n}\sum_i x_i^{(a)} (x_i^{(b)})^\intercal \ \in \ \mathbb{R}^{K\times K} \,,
	\label{MoverlapR}
	\\
	Q_{a,b}^{(p)}&\equiv \lambda^\intercal R_{a,b}^{\circ p}\lambda = \sum_{k,k'}\lambda_k\lambda_{k'}(R_{a,b}^{k,k'})^p  \ \in \mathbb{R}\,,
\end{align}
%
where $R_{a,b}^{\circ p}\equiv ((R_{a,b}^{k,k'})^p)_{k,k'\le K}$ is the componentwise power. The posterior then becomes simply 
%
\begin{align}
dP(x|\widetilde Y,Y)=\frac{1}{{\cal Z}(\widetilde Y,Y)}\prod_{i}dP_0(x_i)\exp\{-{\cal H}_0(x;\widetilde Y(X,\widetilde Z))-{\cal H}_{\rm pert}(x;Y(X,Z))\}\,.	
\end{align}
We denote $\langle -\rangle$ the Gibbs-bracket associated with this perturbed posterior (and associated with the product measure $dP(\cdot\,|\widetilde Y,Y)^{\otimes \infty}$ when applied to i.i.d. replicas $(x^{(a)})$), $\EE$ the joint expectation w.r.t. $(X,\widetilde Y,Y)$ or equivalently w.r.t. the independent random variables $(X,\widetilde Z,Z)$.
%
%
\subsection{Ghiranda-Guerra identity in Bayesian inference} % (fold)
\label{sub:ghiranda_guerra_identity_in_bayesian_inference}
%
In order to derive the GG identity for inference we will test $f=f(X,\{x^{(a)}\}_{a=1}^A)$ against the following scalar quantity (we denote equivalently $x=x^{(1)}$):
%
\begin{align}
{\cal L}^{(p)} \equiv \frac{1}{n}\frac{d{\cal H}_{\rm pert}^{(p)}(x;Y)}{d\gamma_n} = \gamma_n Q_{1,1}^{(p)} -2\gamma_n Q_{0,1}^{(p)}-n^{-\frac{1+p}{2}}\sum_I Z_Ix_{I}^\intercal \lambda\,.
\end{align}
%
Integrating by parts the noise we get
%
\begin{align}
	\EE\langle {\cal L}^{(p)}\rangle = \EE\Big\langle \gamma_n Q_{1,1}^{(p)}-2\gamma_n Q_{0,1}^{(p)}-n^{-\frac{1+p}{2}}\sum_I Z_Ix_{I}^\intercal \lambda\Big\rangle &= \EE\big\langle\gamma_nQ_{1,2}^{(p)}-2\gamma_n Q_{0,1}^{(p)}\big\rangle=-\gamma_n\EE\big\langle Q_{0,1}^{(p)}\big\rangle
\end{align}
%
using the Nishimori identity $\EE\langle Q_{0,1}^{(p)}\rangle = \EE\langle Q_{1,2}^{(p)}\rangle$. 

We now test $f(X,\{x^{(a)}\}_{a=1}^A)$ against ${\cal L}^{(p)}$. We emphasize here the dependence on $X$ which still plays a special role; indeed we cannot use yet the Nishimori identity and consider the signal $X=x^{(0)}$ as another replica, because the Nishimori identity can be applied only to functions depending on replicas and on the observations, not one the noise variables as what appears in ${\cal L}^{(p)}$. We obtain by careful Gaussian integration by parts 
%
\begin{align}
\EE\langle {\cal L}^{(p)}f\rangle	&= \EE\Big\langle \gamma_n Q_{1,1}^{(p)}f-2\gamma_nQ_{0,1}^{(p)}f-n^{-\frac{1+p}{2}}\sum_{I} Z_I\lambda^\intercal x_{I}f\Big\rangle \nn
&=\gamma_n\EE\Big\langle Q_{1,1}^{(p)}f-2Q_{0,1}^{(p)}f-\sum_{a=1}^A Q_{1,a}^{(p)}f+AQ_{1,A+1}^{(p)}f\Big\rangle \nonumber\\
&=\gamma_n\EE\Big\langle AQ_{1,A+1}^{(p)}f-2Q_{0,1}^{(p)}f-\sum_{a=2}^A Q_{1,a}^{(p)}f\Big\rangle \,.
\end{align}
%
At this stage one can now use the Nishimori identity and therefore consider the signal as an ordinary i.i.d. replica, and thus $f(X,\{x^{(a)}\}_{a=1}^A)=f(\{x^{(a)}\}_{a=0}^K)$. Therefore from the concentration of ${\cal L}^{(p)}$ onto $\EE\langle {\cal L}^{(p)}\rangle$ under an $\EE_\beta$ average (that can be proved using a combination of the Nishimori identity, and the convexity of the free energy as well as the concentration of the free energy) we obtain the following modified matrix GG identity for the generalized overlaps in inference:
%
\begin{align}
\lim_{n\to\infty}\EE_\beta \Big|\frac1A \sum_{a=2}^A\EE\langle Q_{1,a}^{(p)}f\rangle - \frac{1}{A} \EE\langle  Q_{0,1}^{(p)}\rangle \EE\langle f\rangle  - \EE\langle Q_{1,A+1}^{(p)}f\rangle+\frac2A\EE\langle Q_{0,1}^{(p)}f\rangle \Big|	=0 \label{GG_inf}
\end{align}
%
for any bounded function $f(\{x^{(a)}\}_{a=0}^A)$ of $A+1$ i.i.d. replicas drawn from the (perturbed) posterior measure.
%
\subsection{Concentration of the generalized overlap}
%
One special case of interest is when whe choose $f(x^{(0)},x^{(1)})=Q_{0,1}^{(p)}$, $A=1$. In this case the identity \eqref{GG_inf} becomes
%
\begin{align}
\lim_{n\to\infty}\EE_\beta \Big|- \EE[\langle  Q_{0,1}^{(p)}\rangle]^2 - \EE\langle Q_{1,2}^{(p)}Q_{0,1}^{(p)}\rangle+2\,\EE\langle (Q_{0,1}^{(p)})^2\rangle \Big|	=0\,.\label{12}
\end{align}
%
This simplifies using the Nishimori identity: Replacing replica $0$ by the signal $X$ one can check
%
\begin{align}
\EE\langle Q_{1,2}^{(p)}Q_{0,1}^{(p)}\rangle=\EE\langle Q_{0,2}^{(p)}Q_{1,0}^{(p)}\rangle=\EE[\langle Q_{0,1}^{(p)}\rangle^2]	\,.
\end{align}
%
Therefore \eqref{12} becomes
%
\begin{align}
\lim_{n\to\infty}\EE_\beta \Big(\big\{\EE\langle (Q_{0,1}^{(p)})^2\rangle- \EE[\langle  Q_{0,1}^{(p)}\rangle]^2\big\} +\big\{\EE\langle(Q_{0,1}^{(p)})^2\rangle- \EE[\langle Q_{0,1}^{(p)}\rangle^2] \big\}\Big)	=0\label{14}
\end{align}
%
i.e. both the thermal and quenched fluctuations of $Q_{0,1}^{(p)}$ vanish: This is why the Nishimori identity prevents replica symmetry breaking to occur. Remark also the following. {\it Assume} that the (generalized) overlap concentrates onto its thermal average (a simple fact to show in Bayesian inference), which means that the second fluctuation $\{\dots\}$ in \eqref{14} vanishes. Identity \eqref{14} then yields that the disorder fluctuations vanish too. Therefore {\it on the Nishimori line and under the perturbation \eqref{one_inf} the thermal concentration directly implies the concentration w.r.t. the quenched disorder.}
%
\subsection{Concentration of the matrix overlap}
%

The proof of an adaptation of the proof of Theorem 3 in \cite{Panchenko_potts}, with some simplifications due to replica symmetry of the overlaps $Q_{\ell,\ell'}$ in (\ref{14}). For convenience of the reader, we will repeat the details. Given $1\leq k\not=k'\leq K,$ let us consider several choices of the overlap $Q_{\ell,\ell'}=Q_{\ell,\ell'}^{\lambda,p}$. 
\begin{enumerate}
\item $Q_{\ell,\ell'}=R_{\ell,\ell'}^{k,k}$ if $p=1$, $\lambda_k=1$, and $\lambda_j=0$ for $j\not = k$.

\item $Q_{\ell,\ell'}=R_{\ell,\ell'}^{k,k}+R_{\ell,\ell'}^{k',k'}+R_{\ell,\ell'}^{k,k'}+R_{\ell,\ell'}^{k',k}$ if $p=1$, $\lambda_k=\lambda_{k'}=1$, and $\lambda_j=0$ for $j\not = k,k'$.

\item $Q_{\ell,\ell'}=(R_{\ell,\ell'}^{k,k})^2+(R_{\ell,\ell'}^{k',k'})^2+(R_{\ell,\ell'}^{k,k'})^2+(R_{\ell,\ell'}^{k',k})^2$ if $p=2$, $\lambda_k=\lambda_{k'}=1$, and $\lambda_j=0$ for $j\not = k,k'$.
\end{enumerate}
The fact that, for $\ell\not=\ell',$ all these overlaps are constants implies that 
$$
R_{\ell,\ell'}^{k,k}=a,\,\, R_{\ell,\ell'}^{k',k'}=d
$$
for some constants $a,d\geq 0$ that may depend on $k,k',$ and, as a result, 
$$
R_{\ell,\ell'}^{k,k'}+R_{\ell,\ell'}^{k',k} = x,
(R_{\ell,\ell'}^{k,k'})^2+(R_{\ell,\ell'}^{k',k})^2 = y,
$$
for some constants $x,y\geq 0$ that may also depend on $k,k'.$  The systems of equations of the form $r+q=x,$ $r^2+q^2=y$ can be solved to find $\{r,q\}$ in terms of $x$ and $y$, 
$$
r,q = \frac{x\pm \sqrt{2y-x^2}}{2}.
$$
In other words, for some constants $b,c$ that may depend on $k,k'$,
$
\bigl\{R_{\ell,\ell'}^{k,k'}, R_{\ell,\ell'}^{k',k} \bigr\} = 
\bigl\{ b,c \bigr\}.
$
This shows that
\begin{equation}
\begin{bmatrix}
R_{\ell,\ell'}^{k,k} & R_{\ell,\ell'}^{k,k'} \\
R_{\ell,\ell'}^{k',k}  & R_{\ell,\ell'}^{k',k'} 
\end{bmatrix}
=
\begin{bmatrix}
a & b \\
c & d
\end{bmatrix}
\,\mbox{ or }\,
\begin{bmatrix}
a & c \\
b & d
\end{bmatrix}
\label{f1f2}
\end{equation}
for all $\ell\not =\ell'$. This still allows for some randomness in the off-diagonal entries $R_{\ell,\ell'}^{k,k'}, R_{\ell,\ell'}^{k',k}$. The remaining argument that allows to show that $b=c$ and, hence, off-diagonal entries are also constant, corresponds to ?? in Panchenko's article.

% We will need the following. Directed complete graphs are called tournaments and, given two tournaments $S$ and $T$, $T$ is called $S$-free if $S$ is not a sub-tournament of $T.$ Theorem 3 in \cite{Erdos} states that if $T$ is $S$-free, $\mathrm{card}(S)=m$ and $\mathrm{card}(T)=n$ then one can find two disjoint subsets $V_1, V_2$ in $T$ of cardinality 
% $$
% \mathrm{card}(V_1) = \mathrm{card}(V_2) =
% \Bigl \lfloor{(n/m)^{1/(m-1)}} \Bigr\rfloor
% $$
% with all edges between them oriented from $V_1$ to $V_2.$  Take $S$ consisting of two groups of cardinality $m$ with edges between groups oriented in one direction, and in arbitrary fashion within groups. If $T$ contains $S$ then is has two subsets $V_1, V_2$ of cardinality $m$ such that all edges between them are oriented from $V_1$ to $V_2.$ If not then, by the above claim, it contains two such subsets of cardinality $\lfloor{(n/2m)^{1/(2m-1)}}\rfloor.$ If we set $(n/2m)^{1/(2m-1)}= m/2$, we find that $m$ is of order $\log n / \log\log n$, which means that, for large $n$, we can always find two large disjoint subsets with edges between them oriented in the same direction.


% Consider a realization of the random array $R_{\ell,\ell'}^{j,j'}$ and, given $n$, define a tournament $(V,E)$ on $n$ vertices such that, for each pair $1\leq \ell\not =\ell'\leq n$, the edge is oriented $\ell\to\ell'$ or $\ell'\to\ell$ depending on whether the first or second option in (\ref{f1f2}) is realized. Let $V_1,V_2\subseteq V=\{1,\ldots, n\}$ be two disjoint subsets of size $m$ as defined above. This means that for all $\ell\in V_1$ and $\ell'\in V_2$,
% $$
% \begin{bmatrix}
% R_{\ell,\ell'}^{k,k} & R_{\ell,\ell'}^{k,k'} \\
% R_{\ell,\ell'}^{k',k}  & R_{\ell,\ell'}^{k',k'} 
% \end{bmatrix}
% =
% \begin{bmatrix}
% a & b \\
% c & d
% \end{bmatrix}.
% $$
% On the other hand, the $2n\times 2n$ array consisting of these $2\times 2$ blocks is positive-semidefinite because, by the definition of overlaps in (\ref{MoverlapR}), it is a limit (in distribution) of Gram matrices. Therefore, we can find pairs of vectors $u_\ell,w_{\ell}$ for $1\leq \ell\leq n$ in a Hilbert space $H$ such that, for all $\ell\not =\ell'$,
% \begin{equation}
% \begin{bmatrix}
% (u_{\ell},u_{\ell'}) & (u_{\ell},w_{\ell'}) \\
% (w_{\ell},u_{\ell'}) & (w_{\ell},w_{\ell'})
% \end{bmatrix}
% =
% \begin{bmatrix}
% a & b \\
% c & d
% \end{bmatrix}
% \,\mbox{ or }\,
% \begin{bmatrix}
% a & c \\
% b & d
% \end{bmatrix}
% \label{Step5eq1}
% \end{equation}
% and, by construction, for all $\ell\in V_1$ and $\ell'\in V_2$,
% \begin{equation}
% \begin{bmatrix}
% (u_{\ell},u_{\ell'}) & (u_{\ell},w_{\ell'}) \\
% (w_{\ell},u_{\ell'}) & (w_{\ell},w_{\ell'})
% \end{bmatrix}
% =
% \begin{bmatrix}
% a & b \\
% c & d
% \end{bmatrix}.
% \label{Step5eq2}
% \end{equation}
% For $j=1,2$, let us consider the barycentres
% $$
% U_j = \frac{1}{m}\sum_{\ell\in V_j} u_\ell
% \,\mbox{ and }\,
% W_j = \frac{1}{m}\sum_{\ell\in V_j} w_\ell. 
% $$
% On the one hand, using the equation (\ref{Step5eq2}),
% $$
% \begin{bmatrix}
% (U_1,U_2) & (U_1,W_2) \\
% (W_1,U_2) & (W_1,W_2)
% \end{bmatrix}
% =
% \begin{bmatrix}
% a & b \\
% c & d
% \end{bmatrix}.
% $$ 
% On the other hand, by (\ref{Step5eq1}), $(u_{\ell},u_{\ell'})=a$ and $(w_{\ell},w_{\ell'})=b$ for all $\ell\not =\ell'$ and, since the self-overlaps are bounded, we must have $\|u_\ell\|,\|w_\ell\|\leq L$ for some constant $L>0.$ Therefore,
% $$
% \|U_1 - U_2\|^2 = \frac{1}{m^2}\Bigl\|\sum_{\ell\in V_1} u_\ell-\sum_{\ell\in V_2} u_\ell\Bigr\|^2
% \leq
% \frac{2(L+a)}{m}
% $$
% and
% $$
% \|W_1 - W_2\|^2 = \frac{1}{m^2}\Bigl\|\sum_{\ell\in V_1} w_\ell-\sum_{\ell\in V_2} w_\ell\Bigr\|^2
% \leq
% \frac{2(L+d)}{m}.
% $$
% For large $m$, this implies that $U_1\approx U_2$ and $W_1\approx W_2$ and, therefore, $(U_1,W_2) \approx (W_1,U_2).$ Letting $m\to \infty$ proves that $b=c$.


% \begin{remark}\rm
% Since the array $(Q_{\ell,\ell'}^{\lambda,1})_{\ell,\ell'\geq 1}$ is positive-semidefinite and replica symmetric for all $\lambda$ included in the perturbation, all off-diagonal entries are non-negative, 
% $$
% Q_{\ell,\ell'}^{\lambda,1} = (R_{\ell,\ell'}\lambda,\lambda)\geq 0,
% $$
% where $R_{\ell,\ell'}=(R_{\ell,\ell'}^{k,k'})_{k,k'\leq K}.$ If we want this overlap matrix to be not only symmetric and concentrate in the thermodynamic limit, but also to be positive definite, we can include countably many perturbations with $\lambda\in (\mathbb{Q}\cap[-1,1])^K.$ 
% \qed
% \end{remark}
% %


==> sections/synchronize.tex <==
%
\section{Concentration of the matrix overlap}
%

The proof of an adaptation of the proof of Theorem 3 in \cite{Panchenko_potts}, with some simplifications due to replica symmetry of the overlaps $Q_{\ell,\ell'}$ in (\ref{14}). For convenience of the reader, we will repeat the details. Given $1\leq k\not=k'\leq K,$ let us consider several choices of the overlap $Q_{\ell,\ell'}=Q_{\ell,\ell'}^{\lambda,p}$. 
\begin{enumerate}
\item $Q_{\ell,\ell'}=R_{\ell,\ell'}^{k,k}$ if $p=1$, $\lambda_k=1$, and $\lambda_j=0$ for $j\not = k$.

\item $Q_{\ell,\ell'}=R_{\ell,\ell'}^{k,k}+R_{\ell,\ell'}^{k',k'}+R_{\ell,\ell'}^{k,k'}+R_{\ell,\ell'}^{k',k}$ if $p=1$, $\lambda_k=\lambda_{k'}=1$, and $\lambda_j=0$ for $j\not = k,k'$.

\item $Q_{\ell,\ell'}=(R_{\ell,\ell'}^{k,k})^2+(R_{\ell,\ell'}^{k',k'})^2+(R_{\ell,\ell'}^{k,k'})^2+(R_{\ell,\ell'}^{k',k})^2$ if $p=2$, $\lambda_k=\lambda_{k'}=1$, and $\lambda_j=0$ for $j\not = k,k'$.
\end{enumerate}
The fact that, for $\ell\not=\ell',$ all these overlaps are constants implies that 
$$
R_{\ell,\ell'}^{k,k}=a,\,\, R_{\ell,\ell'}^{k',k'}=d
$$
for some constants $a,d\geq 0$ that may depend on $k,k',$ and, as a result, 
$$
R_{\ell,\ell'}^{k,k'}+R_{\ell,\ell'}^{k',k} = x,
(R_{\ell,\ell'}^{k,k'})^2+(R_{\ell,\ell'}^{k',k})^2 = y,
$$
for some constants $x,y\geq 0$ that may also depend on $k,k'.$  The systems of equations of the form $r+q=x,$ $r^2+q^2=y$ can be solved to find $\{r,q\}$ in terms of $x$ and $y$, 
$$
r,q = \frac{x\pm \sqrt{2y-x^2}}{2}.
$$
In other words, for some constants $b,c$ that may depend on $k,k'$,
$
\bigl\{R_{\ell,\ell'}^{k,k'}, R_{\ell,\ell'}^{k',k} \bigr\} = 
\bigl\{ b,c \bigr\}.
$
This shows that
\begin{equation}
\begin{bmatrix}
R_{\ell,\ell'}^{k,k} & R_{\ell,\ell'}^{k,k'} \\
R_{\ell,\ell'}^{k',k}  & R_{\ell,\ell'}^{k',k'} 
\end{bmatrix}
=
\begin{bmatrix}
a & b \\
c & d
\end{bmatrix}
\,\mbox{ or }\,
\begin{bmatrix}
a & c \\
b & d
\end{bmatrix}
\label{f1f2}
\end{equation}
for all $\ell\not =\ell'$. This still allows for some randomness in the off-diagonal entries $R_{\ell,\ell'}^{k,k'}, R_{\ell,\ell'}^{k',k}.$ We will now show that $b=c$ and, hence, off-diagonal entries are also constant.

We will need the following. Directed complete graphs are called tournaments and, given two tournaments $S$ and $T$, $T$ is called $S$-free if $S$ is not a sub-tournament of $T.$ Theorem 3 in \cite{Erdos} states that if $T$ is $S$-free, $\mathrm{card}(S)=m$ and $\mathrm{card}(T)=n$ then one can find two disjoint subsets $V_1, V_2$ in $T$ of cardinality 
$$
\mathrm{card}(V_1) = \mathrm{card}(V_2) =
\Bigl \lfloor{(n/m)^{1/(m-1)}} \Bigr\rfloor
$$
with all edges between them oriented from $V_1$ to $V_2.$  Take $S$ consisting of two groups of cardinality $m$ with edges between groups oriented in one direction, and in arbitrary fashion within groups. If $T$ contains $S$ then is has two subsets $V_1, V_2$ of cardinality $m$ such that all edges between them are oriented from $V_1$ to $V_2.$ If not then, by the above claim, it contains two such subsets of cardinality $\lfloor{(n/2m)^{1/(2m-1)}}\rfloor.$ If we set $(n/2m)^{1/(2m-1)}= m/2$, we find that $m$ is of order $\log n / \log\log n$, which means that, for large $n$, we can always find two large disjoint subsets with edges between them oriented in the same direction.


Consider a realization of the random array $R_{\ell,\ell'}^{j,j'}$ and, given $n$, define a tournament $(V,E)$ on $n$ vertices such that, for each pair $1\leq \ell\not =\ell'\leq n$, the edge is oriented $\ell\to\ell'$ or $\ell'\to\ell$ depending on whether the first or second option in (\ref{f1f2}) is realized. Let $V_1,V_2\subseteq V=\{1,\ldots, n\}$ be two disjoint subsets of size $m$ as defined above. This means that for all $\ell\in V_1$ and $\ell'\in V_2$,
$$
\begin{bmatrix}
R_{\ell,\ell'}^{k,k} & R_{\ell,\ell'}^{k,k'} \\
R_{\ell,\ell'}^{k',k}  & R_{\ell,\ell'}^{k',k'} 
\end{bmatrix}
=
\begin{bmatrix}
a & b \\
c & d
\end{bmatrix}.
$$
On the other hand, the $2n\times 2n$ array consisting of these $2\times 2$ blocks is positive-semidefinite because, by the definition of overlaps in (\ref{MoverlapR}), it is a limit (in distribution) of Gram matrices. Therefore, we can find pairs of vectors $u_\ell,w_{\ell}$ for $1\leq \ell\leq n$ in a Hilbert space $H$ such that, for all $\ell\not =\ell'$,
\begin{equation}
\begin{bmatrix}
(u_{\ell},u_{\ell'}) & (u_{\ell},w_{\ell'}) \\
(w_{\ell},u_{\ell'}) & (w_{\ell},w_{\ell'})
\end{bmatrix}
=
\begin{bmatrix}
a & b \\
c & d
\end{bmatrix}
\,\mbox{ or }\,
\begin{bmatrix}
a & c \\
b & d
\end{bmatrix}
\label{Step5eq1}
\end{equation}
and, by construction, for all $\ell\in V_1$ and $\ell'\in V_2$,
\begin{equation}
\begin{bmatrix}
(u_{\ell},u_{\ell'}) & (u_{\ell},w_{\ell'}) \\
(w_{\ell},u_{\ell'}) & (w_{\ell},w_{\ell'})
\end{bmatrix}
=
\begin{bmatrix}
a & b \\
c & d
\end{bmatrix}.
\label{Step5eq2}
\end{equation}
For $j=1,2$, let us consider the barycentres
$$
U_j = \frac{1}{m}\sum_{\ell\in V_j} u_\ell
\,\mbox{ and }\,
W_j = \frac{1}{m}\sum_{\ell\in V_j} w_\ell. 
$$
On the one hand, using the equation (\ref{Step5eq2}),
$$
\begin{bmatrix}
(U_1,U_2) & (U_1,W_2) \\
(W_1,U_2) & (W_1,W_2)
\end{bmatrix}
=
\begin{bmatrix}
a & b \\
c & d
\end{bmatrix}.
$$ 
On the other hand, by (\ref{Step5eq1}), $(u_{\ell},u_{\ell'})=a$ and $(w_{\ell},w_{\ell'})=b$ for all $\ell\not =\ell'$ and, since the self-overlaps are bounded, we must have $\|u_\ell\|,\|w_\ell\|\leq L$ for some constant $L>0.$ Therefore,
$$
\|U_1 - U_2\|^2 = \frac{1}{m^2}\Bigl\|\sum_{\ell\in V_1} u_\ell-\sum_{\ell\in V_2} u_\ell\Bigr\|^2
\leq
\frac{2(L+a)}{m}
$$
and
$$
\|W_1 - W_2\|^2 = \frac{1}{m^2}\Bigl\|\sum_{\ell\in V_1} w_\ell-\sum_{\ell\in V_2} w_\ell\Bigr\|^2
\leq
\frac{2(L+d)}{m}.
$$
For large $m$, this implies that $U_1\approx U_2$ and $W_1\approx W_2$ and, therefore, $(U_1,W_2) \approx (W_1,U_2).$ Letting $m\to \infty$ proves that $b=c$.


\begin{remark}\rm
Since the array $(Q_{\ell,\ell'}^{\lambda,1})_{\ell,\ell'\geq 1}$ is positive-semidefinite and replica symmetric for all $\lambda$ included in the perturbation, all off-diagonal entries are non-negative, 
$$
Q_{\ell,\ell'}^{\lambda,1} = (R_{\ell,\ell'}\lambda,\lambda)\geq 0,
$$
where $R_{\ell,\ell'}=(R_{\ell,\ell'}^{k,k'})_{k,k'\leq K}.$ If we want this overlap matrix to be not only symmetric and concentrate in the thermodynamic limit, but also to be positive definite, we can include countably many perturbations with $\lambda\in (\mathbb{Q}\cap[-1,1])^K.$ 
\qed
\end{remark}
%





==> sections/total_better.tex <==
\subsection{Total fluctuations: proof of Theorem~\ref{thm:Q_con}}
%
Now that we control the thermal fluctuations we are in position to prove the main Theorem~\ref{thm:Q_con}, which shows that the overlap not only concentrates w.r.t. the posterior distribution, but also w.r.t. the quenched variables. The spirit of the proof is similar to the derivation of the Ghirlanda-Guerra identities in the context of spin glasses \cite{GhirlandaGuerra:1998}. Our goal here is to compute (consider first $l\neq l'$)
%
\begin{align}
\EE_\lambda\EE \big\langle Q_{ll'}({\cal L}_{ll'} -\EE\langle {\cal L}_{ll'}\rangle)\big \rangle &=\EE_\lambda\EE \langle Q_{ll'}{\cal L}_{ll'}\rangle + \EE_\lambda \EE\big[\langle Q_{ll'}\rangle^2\big]\,, \label{103easy}
\end{align}
%
using that $\EE\langle {\cal L}\rangle = \frac12 {\rm diag}(\EE\langle Q\rangle)-\EE\langle Q\rangle$ by \eqref{80}, \eqref{80_ll}, and that $\EE \langle Q\rangle$ is symmetric. The crux of the proof is that $\EE_\lambda{\rm Tr}\,\EE \langle Q({\cal L} -\EE\langle {\cal L}\rangle)\rangle$ will make appear the fluctuations of the overlap, and is small by Proposition~\ref{prop:Lconc} (with Cauchy-Schwarz).

It thus only remains to compute $\EE_\lambda{\rm Tr}\,\EE \langle Q{\cal L}\rangle$. Let us first consider the off-diagonal terms:
%
\begin{align}
\sum_{l\neq l'} \EE_\lambda\EE \langle Q_{ll'}{\cal L}_{l'l}\rangle &=\sum_{l\neq l'} \EE_\lambda\EE\Big[ \frac{1}{n}\sum_{i=1}^n \langle Q_{ll'} x_{il} x_{il'}\rangle -\langle Q_{ll'}Q_{l'l}\rangle -\langle Q_{ll'}^2\rangle -   \frac{1}{n}\sum_{i=1}^n\Big\langle Q_{ll'} x_{i}^\intercal \frac{d\lambda^{1/2}}{d\lambda_{ll'}} \, Z_{i}\Big\rangle\Big]\,.\label{32}
\end{align}
%
We need to simplify the last term. Using \eqref{77},
%
\begin{align}
\EE_\lambda\EE\Big\langle Q_{ll'} x_{i}^\intercal \frac{d\lambda^{1/2}}{d\lambda_{ll'}} \, Z_{i}\Big\rangle &=	\EE_\lambda\EE\Big[\Big\langle Q_{ll'}x_i^\intercal\frac{d\lambda^{1/2}}{d\lambda_{ll'}} \lambda^{1/2} x_i  \Big\rangle - \langle Q_{ll'}x_i^\intercal\rangle\frac{d\lambda^{1/2}}{d\lambda_{ll'}} \lambda^{1/2} \langle x_i\rangle \Big]\nn
%
&=\EE_\lambda\EE\Big[\langle Q_{ll'}x_{il}x_{il'}  \rangle - \langle Q_{ll'}x_i^\intercal\rangle\frac{d\lambda^{1/2}}{d\lambda_{ll'}} \lambda^{1/2} \langle x_i\rangle \Big]\,.\label{33}
\end{align}
%
The first term has been simplified because $x_ix_i^\intercal$ is symmetric, allowing the symmetrization of $\frac{d\lambda^{1/2}}{d\lambda_{ll'}}$ followed by the use of \eqref{57}. In contrast the second term above lacks symmetry as the matrix $\langle x_i\rangle \langle Q_{ll'} x_i^\intercal\rangle$ is not symmetric. This prevents the use of the mechanism employed for the first term. In order to face this issue we exploit the concentration of the overlap w.r.t. the posterior. We can write
%
\begin{align*}
\Big|\EE_\lambda\EE\Big[\langle Q_{ll'}x_i^\intercal\rangle\frac{d\lambda^{1/2}}{d\lambda_{ll'}} \lambda^{1/2} \langle x_i\rangle \Big]	- \EE_\lambda\EE\Big[\langle Q_{ll'}\rangle \langle x_i\rangle^\intercal\frac{d\lambda^{1/2}}{d\lambda_{ll'}} \lambda^{1/2} \langle x_i\rangle \Big]\Big| \le  \frac{C(K,S)}{(s_nn)^{1/4}}
\end{align*}
%
by relation \eqref{36} in Proposition~\ref{prop:thermalBOund} and Cauchy-Schwarz, because the entries of the matrix $\frac{d\lambda^{1/2}}{d\lambda_{ll'}} \lambda^{1/2}$ are bounded as well as the support of the prior (so $|\langle x_{ik}\rangle|\le S$). Now we can exploit symmetry and therefore write
%
\begin{align*}
\EE_\lambda\EE\Big[\langle Q_{ll'}\rangle \langle x_i\rangle^\intercal\frac{d\lambda^{1/2}}{d\lambda_{ll'}} \lambda^{1/2} \langle x_i\rangle \Big]&=\frac12\EE_\lambda\EE\Big[\langle Q_{ll'}\rangle \langle x_i\rangle^\intercal\Big\{\frac{d\lambda^{1/2}}{d\lambda_{ll'}} \lambda^{1/2}+\lambda^{1/2}\frac{d\lambda^{1/2}}{d\lambda_{ll'}} \Big\} \langle x_i\rangle \Big]	\nn
&=\frac12\EE_\lambda\EE\Big[\langle Q_{ll'}\rangle \langle x_i\rangle^\intercal\frac{d\lambda}{d\lambda_{ll'}} \langle x_i\rangle \Big]=\EE_\lambda\EE\big[\langle Q_{ll'}\rangle \langle x_{il}\rangle\langle x_{il'}\rangle \big]\,.
\end{align*}
%
Combining everything in \eqref{33} and \eqref{32} yields
%
\begin{align*}
\sum_{l\neq l'} \EE_\lambda\EE \langle Q_{ll'}{\cal L}_{l'l}\rangle &=\sum_{l\neq l'} \EE_\lambda\EE\Big[-\langle Q_{ll'}Q_{l'l}\rangle -\langle Q_{ll'}^2\rangle +\langle Q_{ll'}\rangle\langle Q_{ll'}^{(12)}\rangle \Big]+{\cal O}_{K,S}((s_nn)^{-1/4})
\end{align*}
%
using $Q^{(12)}_{ll'}\equiv \frac1n \sum_{i=1}^n x_{il}^{(1)}x_{il'}^{(2)}$ and thus $\langle Q^{(12)}_{ll'}\rangle \equiv \frac1n \sum_{i=1}^n \langle x_{il}\rangle \langle x_{il'}\rangle$ (which is symmetric). The notation $A=B+{\cal O}_{K,S}((s_nn)^{-1/4})$ means $|A-B|\le C(K,S)(s_nn)^{-1/4}$. We now consider the diagonal terms. Similarly
%
\begin{align*}
\sum_{l} \EE_\lambda\EE \langle Q_{ll}{\cal L}_{ll}\rangle &= \sum_{l} \EE_\lambda\EE\Big[ \frac{1}{2n}\sum_{i=1}^n  \langle Q_{ll}x_{il}^2\rangle -\langle Q_{ll}^2\rangle  - \frac{1}{n}\sum_{i=1}^n \Big \langle Q_{ll}x_{i}^\intercal \frac{d\lambda^{1/2}}{d\lambda_{ll}} \, {Z}_{i}  \Big\rangle\Big]\nonumber\\
%
&=\sum_{l}\EE_\lambda\EE\Big[   -\langle Q_{ll}^2\rangle +\frac12\langle Q_{ll}\rangle \langle Q_{ll}^{(12)}\rangle\Big]+{\cal O}_{K,S}((s_nn)^{-1/4})\,.
%
\end{align*}
%
Summing everything we obtain
%
\begin{align*}
\EE_\lambda{\rm Tr}\,\EE \langle Q{\cal L}\rangle&=\sum_{l,l'}\EE_\lambda\EE\Big[\langle Q_{ll'}\rangle \langle Q_{ll'}^{(12)}\rangle-\langle Q_{ll'}Q_{l'l}\rangle -\langle Q_{ll'}^2\rangle \Big]\nn
&\qquad\qquad\qquad+\sum_{l}\EE_\lambda\EE\Big[\langle Q_{ll}^2\rangle - \frac12 \langle Q_{ll}\rangle\langle Q_{ll}^{(12)}\rangle\Big]+{\cal O}_{K,S}((s_nn)^{-1/4})\nonumber\\
%
&= \EE_\lambda{\rm Tr}\,\EE\big[\langle Q\rangle\langle Q^{(12)}\rangle\big]-\EE_\lambda{\rm Tr}\,\EE\langle Q^2\rangle -\EE_\lambda\EE\big\langle\| Q \|_{\rm F}^2\big\rangle \nn
&\qquad\qquad\qquad+ \sum_{l}\EE_\lambda\EE\Big[\langle Q_{ll}^2\rangle - \frac12 \langle Q_{ll}\rangle\langle Q_{ll}^{(12)}\rangle\Big]+{\cal O}_{K,S}((s_nn)^{-1/4})\,. 
\end{align*}
%
Therefore, plugging this in \eqref{103easy} leads to
%
\begin{align*}
\EE_\lambda{\rm Tr}\,\EE \big\langle &Q({\cal L} -\EE\langle {\cal L}\rangle) \big\rangle	= -\EE_\lambda\EE\big\langle\| Q \|_{\rm F}^2\big\rangle+ \EE_\lambda\big[\| \EE\langle Q\rangle\|_{\rm F}^2\big]+ \frac12\sum_{l}\EE_\lambda\big[\EE\langle Q_{ll}^2\rangle-\EE[\langle Q_{ll}\rangle]^2\big] \nn
& +\EE_\lambda{\rm Tr}\,\EE\big\langle Q(\langle Q^{(12)}\rangle -Q)\big\rangle+ \EE_\lambda\EE\big\langle Q_{ll}(Q_{ll}- \langle Q_{ll}^{(12)}\rangle)\big\rangle+{\cal O}_{K,S}((s_nn)^{-1/4})\,.
\end{align*}	
%
A direct application of \eqref{2terms_controlled} in Proposition~\ref{prop:thermalBOund} together with Cauchy-Schwarz gives:
%
\begin{align*}
\big|\EE_\lambda{\rm Tr}\,\EE\big\langle Q(\langle Q^{(12)}\rangle -Q)\big\rangle\big|\le \Big\{\EE_\lambda\EE\big\langle \|Q\|_{\rm F}^{2}\big\rangle\, \EE_\lambda\EE\big\langle \| Q-\langle Q^{(12)}\rangle\|_{\rm F}^2\big\rangle\Big\}^{1/2}	\le \frac{C(K,S)}{(s_nn)^{1/4}}
\end{align*}
%
as the overlap is bounded by some $C(S)$. Similarly $\big|\EE_\lambda\EE\big\langle Q_{ll}(Q_{ll}- \langle Q_{ll}^{(12)}\rangle)\big\rangle\big| \le \frac{C(K,S)}{(s_nn)^{1/4}}$. Therefore
%
\begin{align}
\EE_\lambda{\rm Tr}\,\EE \big\langle Q({\cal L} -\EE\langle {\cal L}\rangle) \big\rangle	&= -2\sum_{l>l'}\EE_\lambda\EE\big\langle (Q_{ll'}-\EE\langle Q_{ll'}\rangle)^2\big\rangle - \frac12\sum_{l}\EE_\lambda\EE\big\langle (Q_{ll}-\EE\langle Q_{ll}\rangle)^2\big\rangle \nn
&\qquad\qquad\qquad\qquad+{\cal O}_{K,S}((s_nn)^{-1/4})\,.\label{47}
\end{align}
%
Finally by Cauchy-Schwarz and Proposition~\ref{prop:Lconc} we are allowed to write
%
\begin{align*}
 \big|\EE_\lambda{\rm Tr}\,\EE \big\langle Q({\cal L} -\EE\langle {\cal L}\rangle) \big\rangle\big| &\le 	C(S) \Big\{\EE_\lambda\EE\big\langle \|{\cal L} -\EE\langle {\cal L}\rangle\|_{\rm F}^2\big\rangle\Big\}^{1/2} \le \frac{C(C_f,K,S)}{(s_n^{4}n)^{1/6}}\,.
\end{align*}
%
 This inequality combined with \eqref{47} gives
 %
 \begin{align*}
 2\sum_{l>l'}\EE_\lambda\EE\big\langle (Q_{ll'}-\EE\langle Q_{ll'}\rangle)^2\big\rangle + \frac12\sum_{l}\EE_\lambda\EE\big\langle (Q_{ll}-\EE\langle Q_{ll}\rangle)^2\big\rangle\le \frac{C(C_f,K,S)}{(s_n^{4}n)^{1/6}}	
 \end{align*}
 and thus the final result Theorem~\ref{thm:Q_con}. $\QED$
